Is There an Analog of Nesterov Acceleration for MCMC?

We formulate gradient-based Markov chain Monte Carlo (MCMC) sampling as optimization on the space of probability measures, with Kullback-Leibler (KL) divergence as the objective functional. We show that an underdamped form of the Langevin algorithm performs accelerated gradient descent in this metric. To characterize the convergence of the algorithm, we construct a Lyapunov functional and exploit hypocoercivity of the underdamped Langevin algorithm. As an application, we show that accelerated rates can be obtained for a class of nonconvex functions with the Langevin algorithm.

==> continuous.tex <==
\subsection{Continuous Underdamped Langevin Diffusion Dynamics}
Now we consider underdamped Langevin diffusion.
Let the phase space $x_t=(\theta_t, r_t)$ and $\p^*(x) = \p^*(\theta) \p^*(r) = \exp\left( - U(\theta) - \frac{\xi}{2} ||r||_2^2 \right)$.
Then the dynamics can be written as:
\begin{equation}
\left\{
\begin{array}{l}
d \theta_t = \xi r_t d t\\
d r_t = -\gamma \xi r_t d t - \nabla U(\theta_t) d t + \sqrt{2 \gamma} d B_t
\end{array}
\right. . \label{e:underdamp_diff}
\end{equation}
Here,
$D(x)=\left(
\begin{array}{cc}
0 & 0\\
0 & \gamma I
\end{array}
\right)$
and
$Q(x)=\left(
\begin{array}{cc}
0 & - I\\
I & 0
\end{array}
\right)$
and the vector flow is
\begin{align}
v_t
=& -(D(x) + Q(x))\nabla \ln\lrp{\frac{\p_t(x)}{\p^*(x)}} \nonumber\\
=& \left(
\begin{array}{l}
\nabla_r\ln\frac{\p_t(\theta_t, r_t)}{ \p^*(\theta_t, r_t) }\\
- \nabla_\theta\ln\frac{\p_t(\theta_t, r_t)}{ \p^*(\theta_t, r_t) } -\gamma\nabla_r\ln\frac{\p_t(\theta_t, r_t)}{ \p^*(\theta_t, r_t) }
\end{array}
\right) \nonumber\\
=& \left(
\begin{array}{l}
\nabla_r\ln{\p_t(\theta_t, r_t)} + \xi r_t\\
- \nabla_\theta\ln{\p_t(\theta_t, r_t)} - \nabla U(\theta_t) -\gamma\nabla_r\ln\frac{\p_t(\theta_t, r_t)}{ \p^*(r_t) }
\end{array}
\right),
\end{align}
which is equivalent to
\begin{align}
v_t
= \left(
\begin{array}{l}
\xi r_t\\
- \nabla U(\theta_t) -\gamma\nabla_r\ln\frac{\p_t(\theta_t, r_t)}{ \p^*(r_t) }
\end{array}
\right). \label{eq:simple_irr}
\end{align}
